Detecting Grouped Local Average Treatment Effects and Selecting True Instruments

Under an endogenous binary treatment with heterogeneous effects and multiple instruments, we propose a two-step procedure for identifying complier groups with identical local average treatment effects (LATE) despite relying on distinct instruments, even if several instruments violate the identifying assumptions. We use the fact that the LATE is homogeneous for instruments which (i) satisfy the LATE assumptions (instrument validity and treatment monotonicity in the instrument) and (ii) generate identical complier groups in terms of treatment propensities given the respective instruments. We propose a two-step procedure, where we first cluster the propensity scores in the first step and find groups of IVs with the same reduced form parameters in the second step. Under the plurality assumption that within each set of instruments with identical treatment propensities, instruments truly satisfying the LATE assumptions are the largest group, our procedure permits identifying these true instruments in a data driven way. We show that our procedure is consistent and provides consistent and asymptotically normal estimators of underlying LATEs. We also provide a simulation study investigating the finite sample properties of our approach and an empirical application investigating the effect of incarceration on recidivism in the US with judge assignments serving as instruments.

==> Sim_first_step_class_CARDS.tex <==
Setting & Inv. & Method & \#clubs & \#corr & Hansen p & Power & Cover & NMI \\
\midrule
\multirow{2}{*}{20} & \multirow{6}{*}{no} & Oracle & 3 & 1 & 0.50 & 0.99 & 0.95 & 1 \\ %
& & CARDS & 2.33 & 0.33 & 0.50 & 0.86 & 0.95 & 0.65 \\ %
\multirow{2}{*}{60} & & Oracle & 3 & 1 & 0.49 & 1 & 0.95 & 1 \\
& & CARDS & 2.98 & 0.95 & 0.50 & 0.98 & 0.95 & 0.93 \\
\multirow{2}{*}{100} & & Oracle & 3 & 1 & 0.49 & 1 & 0.95 & 1 \\
& & CARDS & 3.01 & 0.99 & 0.49 & 1 & 0.95 & 0.98 \\
\hline
\multirow{2}{*}{20} & \multirow{6}{*}{yes} & Oracle & 3 & 1 & 0.01 & 0.99 & 0.38 %0.93 
& 1 \\
& & CARDS & 2.33 & 0.33 & 0.05 & 0.82 & 0.71 & 0.64 \\
\multirow{2}{*}{60} & & Oracle & 3 & 1 & 0.00 & 1 & 0.27 %0.91 
& 1 \\
& & CARDS & 2.98 & 0.96 & 0.00 & 0.99 & 0.34 & 0.95 \\
\multirow{2}{*}{100} & & Oracle & 3 & 1 & 0.00 & 1 & 0.24 & 1 \\
& & CARDS & 3.02 & 0.98 & 0.00 & 1 & 0.29 & 0.98 \\
   \bottomrule
   


==> Sim_second_step_class_CARDS.tex <==
Setting & Method & Hansen p & Power & Cover & ValDet & InvDet & CorVal \\
\midrule
\multirow{2}{*}{20} & Oracle & 0.51 & 0.96 & 0.94 & 1 & 1 & 1 \\
& CARDS & 0.29 & 0.71 & 0.77 & 0.97 & 0.70 & 0.34 \\
\multirow{2}{*}{60} & Oracle & 0.49 & 1 & 0.95 & 1 & 1 & 1 \\
& CARDS & 0.43 & 0.97 & 0.84 & 0.98 & 0.94 & 0.81 \\
\multirow{2}{*}{100} & Oracle & 0.50 & 1 & 0.95 & 1 & 1 & 1 \\
& CARDS & 0.48 & 0.99 & 0.90 & 0.99 & 0.97 & 0.92 \\
   \bottomrule

==> TableBaseline.tex <==
\begin{tabularx}{1.05\textwidth}{cXXXXXX}
          &\multicolumn{1}{c}{OLS}&\multicolumn{1}{c}{TSLS}&\multicolumn{1}{c}{OLS}&\multicolumn{1}{c}{TSLS}&\multicolumn{1}{c}{OLS}&\multicolumn{1}{c}{TSLS}\\

\midrule D&    0.068&    0.054&    0.061&    0.051&    0.060&    0.033\\
          & (0.0068)&  (0.021)& (0.0096)&  (0.025)&  (0.013)&  (0.028)\\

MinC      &       50&       50&      200&      200&      300&      300\\
N         &    44520&    44520&    23958&    23958&    11219&    11219\\
P         &         &     0.00&         &     0.00&         &     0.00\\
F         &         &    18.53&         &    33.44&         &    76.50\\
\bottomrule \end{tabularx}


==> firststage_baseline.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% TueMon Jan 117 16:19:582:31:22 2022
\begin{tabular}{lllllll}
 Variable & Coef. & (p-Value) & Sign. Level & F-Statistic & (p-Value) & Sign. Level \\ 
  \midrule
A. No Control &  &  &  &  &  &  \\ 
  Judge Stringency & 0.9635 & (0) & *** & 1981.388 & (0) & *** \\ 
  Judge Dummies &  &  &  & 15.1904 & (0) & *** \\ 
   \midrule
B. Court x Year FE &  &  &  &  &  &  \\ 
  Judge Stringency & 0.6854 & (1.11e-09) & *** & 37.1342 & (1.11e-09) & *** \\ 
  Judge Dummies &  &  &  & 4.553 & (1.16e-93) & *** \\ 
   \midrule
C. Only Covariates &  &  &  &  &  &  \\ 
  Judge Stringency & 0.9492 & (0) & *** & 3318.6578 & (0) & *** \\ 
  Judge Dummies &  &  &  & 15.0684 & (0) & *** \\ 
  D. Covariates \& Court  $\times$x Year FE &  &  &  &  &  &  \\ 
  Judge Stringency & 0.6835 & (1.03e-08) & *** & 32.7912 & (1.03e-08) & *** \\ 
  Judge Dummies &  &  &  & 4.6013 & (2.43e-95) & *** \\ 
  \end{tabular}


==> iv_baseline.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Mon Jan 17 12:10:47 2022

\begin{tabular}{llllll}
  \toprule
& Coef. & Standard Error & Sign. Level & Sargan-J & p-val. \\ 
  \midrule
OLS: No Controls & 0.0815 & 0.008 & *** &  &  \\ 
  OLS: Only Court x Year FE & 0.077 & 0.009 & *** &  &  \\ 
  OLS: Only Covariates & 0.0674 & 0.008 & *** &  &  \\ 
  OLS: Covariates \& Court x Year FE & 0.0701 & 0.009 & *** &  &  \\ 
  IV Stringency: No Controls & 0.092 & 0.022 & *** &  &  \\ 
  IV Stringency: Only Court x Year FE & 0.0744 & 0.083 &   &  &  \\ 
  IV Stringency: Only Covariates & 0.0541 & 0.022 & * &  &  \\ 
  IV Stringency: Covariates \& Court x Year FE & 0.0995 & 0.095 &   &  &  \\ 
  IV Judge Dummies: No Controls & 0.0578 & 0.041 &   & 409.16 & 0 \\ 
  IV Judge Dummies: Only Court x Year FE & 0.02 & 0.048 &   & 233.28 & 0.001 \\ 
  IV Judge Dummies: Only Covariates & 0.0431 & 0.038 &   & 358.96 & 0 \\ 
  IV Judge Dummies: Covariates \& Court x Year FE & 0.0538 & 0.055 &   & 216.55 & 0.012 \\ 
   \bottomrule
\end{tabular}


